A Deep Perceptual Measure for Lens and Camera Calibration

Image editing and compositing have become ubiquitous in entertainment, from digital art to AR and VR experiences. To produce beautiful composites, the camera needs to be geometrically calibrated, which can be tedious and requires a physical calibration target. In place of the traditional multi-image calibration process, we propose to infer the camera calibration parameters such as pitch, roll, field of view, and lens distortion directly from a single image using a deep convolutional neural network. We train this network using automatically generated samples from a large-scale panorama dataset, yielding competitive accuracy in terms of standard `2 error. However, we argue that minimizing such standard error metrics might not be optimal for many applications. In this work, we investigate human sensitivity to inaccuracies in geometric camera calibration. To this end, we conduct a large-scale human perception study where we ask participants to judge the realism of 3D objects composited with correct and biased camera calibration parameters. Based on this study, we develop a new perceptual measure for camera calibration and demonstrate that our deep calibration network outperforms previous single-image based calibration methods both on standard metrics as well as on this novel perceptual measure. Finally, we demonstrate the use of our calibration network for several applications, including virtual object insertion, image retrieval, and compositing. A demonstration of our approach is available at https://lvsn.github.io/deepcalib .

==> sec_ack.tex <==
%!TEX root = main.tex
\ifCLASSOPTIONcompsoc
   % The Computer Society usually uses the plural form
 \section*{Acknowledgments}
\else
   % regular IEEE prefers the singular form
 \section*{Acknowledgment}
\fi
% FROM CVMP 2019
% This research was partially supported by the KAIST High Risk High Return Project (HRHRP) and KAIST Research Promotion Team through URP program.
% It was also partially supported by the National Research Foundation of Korea (NRF) grant funded by the Korean government (MSIT) (No. NRF-2017R1C1B5077030).
% F. Rameau was supported by Korea Research Fellowship Program through the National Research Foundation of Korea (NRF) funded by the Ministry of Science, ICT and Future Planning (2015H1D3A1066564).
% We are very grateful to Michel Antunes and Jo{\~{a}}o P. Barreto for running their line-based method on our image dataset. We also thank Amirsaman Ashtari for the drone image acquisition.



This research was partially funded by the NSERC Discovery Grant RGPIN-2014-05314, the Korea NRF grant NRF-2017R1C1B5077030, an NSERC USRA to Dominique Pich\'{e}-Meunier, generous gift funding from Adobe to JC Bazin and JF Lalonde, and Nvidia who donated GPUs. 

%
We are grateful to Michel Antunes and Jo{\~{a}}o P. Barreto for running their line-based method on our image dataset. 
%


==> sec_analysis.tex <==




==> sec_dataset.tex <==

\section{Dataset}
\label{sec:dataset}


% Déplacer la figure
\begin{figure}
  \centering
  % \includegraphics[draft,width=\textwidth]{dataset generation}
  \caption{Dataset generation pipeline.}
  \label{fig:dataset_generation}
\end{figure}



==> sec_method.tex <==

\section{Human Perception}
\label{sec:proposed_method}

\begin{figure}
  \centering
  % \includegraphics[draft,width=\textwidth]{architecture}
  \caption{Architecture.}
  \label{fig:architecture}
\end{figure}









==> styles.tex <==


\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\defe.g.,{e.g\onedot} \defe.g.,{{E.g}\onedot}
\defi.e.,{i.e\onedot} \defi.e.,{{I.e}\onedot}
\def\cf{c.f\onedot} \def\Cf{{C.f}\onedot}
\def\etc{etc\onedot} \def\vs{{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{et al\onedot}
\def\aka{a.k.a\onedot}
% \defi.e.,{\emph{i.e}\onedot} \defi.e.,{{I.e}\onedot}
% \defe.g.,{\emph{e.g}\onedot} \defe.g.,{{E.g}\onedot}
%
% \defe.g.,{\emph{e.g}\onedot} \defe.g.,{{E.g}\onedot}
% \defi.e.,{\emph{i.e}\onedot} \defi.e.,{{I.e}\onedot}
% \def\cf{\emph{c.f}\onedot} \def\Cf{{C.f}\onedot}
% \def\etc{\emph{etc}\onedot} \def\vs{{vs}\onedot}
% \def\wrt{\emph{w.r.t}\onedot} \def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
% \def\aka{\emph{a.k.a}\onedot}

%\newcommand{\argmax}{\operatornamewithlimits{argmax}}
%\newcommand{\argmin}{\operatornamewithlimits{argmin}}

\newcommand{\rank}{\mathrm{rank}}
\renewcommand{\vec}{\mathrm{vec}}
\renewcommand{\exp}{\mathrm{exp}}
\def\Vec#1{\mbox{\boldmath $#1$}}
\newcommand{\degree}{\ensuremath{^\circ}}

\newcommand{\inquote}[1]{"#1"} % or ``xx"

\newcommand{\versus}{v.s } % v.s

\newcommand\MyBox[2]{
  \fbox{\lower0.75cm
    \vbox to 1.7cm{\vfil
      \hbox to 1.7cm{\hfil\parbox{1.4cm}{#1\\#2}\hfil}
      \vfil}%
  }%
}

\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{eq.~\ref}[1]{Eq.~(\ref{#1})}
\newcommand{\Sysref}[1]{system~(\ref{#1})}
\newcommand{\Fref}[1]{Fig.~\ref{#1}}
\newcommand{\FCref}[1]{Chapter.~\ref{#1}}
\newcommand{\Cref}[1]{Chap.~\ref{#1}}
\newcommand{sec.~\ref}[1]{Sec.~\ref{#1}}
\newcommand{\Aref}[1]{Alg.~\ref{#1}}
%
\newcommand{\SecRef}[1]{sec.~\ref{#1}}
\newcommand{fig.~\ref}[1]{\Fref{#1}}

\newcommand{\shortcite}[1]{\cite{#1}}

\newcommand{\paragraph}[1]{\textbf{#1}}

\newcommand{\diffCVMPJC}[1]{\textcolor{magenta}{#1}}
\newcommand{\todo}[1]{\textcolor{red}{$<$TODO: #1$>$}}
\newcommand{\todojc}[1]{\textcolor{red}{$<$TODO (from JC): #1$>$}}
\newcommand{\todojcself}[1]{\textcolor{blue}{$<$TODO (from/to JC): #1$>$}}
\newcommand{\totai}{\textcolor{blue}{To Dr. Tai; }}
\newcommand{\towifp}{\textcolor{cyan}{To Dr. Wipf; }}
\newcommand{\comjc}[1]{\textcolor{blue}{$<$JC: #1$>$}}
\newcommand{\joo}[1]{\textcolor{red}{Joo$>$ #1}}
\newcommand{\kim}[1]{\textcolor{cyan}{Kim$>$ #1}}

\newcommand{\tai}[1]{\textcolor{blue}{Tai$>$ #1}}
\newcommand{\wifp}[1]{\textcolor{cyan}{Wipf$>$ #1}}
%%
%\newcommand{\jc}[1]{\textcolor{cyan}{JC$>$ #1}}
\newcommand{\jcrev}[1]{\textcolor{cyan}{#1}}
\newcommand{\joorev}[1]{\textcolor{red}{#1}}


\newcommand{\MMF}{\texttt{MMF}}
\newcommand{\RTMF}{\texttt{RTMF}}
\newcommand{\RMFE}{\texttt{RMFE}}
\newcommand{\vRTMF}{\texttt{vMF-RTMF}}
\newcommand{\aRTMF}{\texttt{approx.-RTMF}}
\newcommand{\eBnB}{\texttt{exhaustive BnB}}
\newcommand{\EBnB}{\texttt{Exhaustive BnB}}
\newcommand{\MPE}{\texttt{MPE}}
\newcommand{\ES}{\texttt{ES}}

\newcommand{\RANSAC} {{\small{RANSAC~}}}
\newcommand{\RANSACnospace} {{\small{RANSAC}}}
\newcommand{\RGBD} {{$\textnormal{RGB-D}$}~}
\newcommand{\RGBDnospace} {{$\textnormal{RGB-D}$}}
\newcommand{\hahe} {{HAHE360~}}

